Electromagnetic Backgrounds and Potassium-42 Activity in the DEAP-3600 Dark Matter Detector

The DEAP-3600 experiment is searching for WIMP dark matter with a 3.3 tonne single phase liquid argon (LAr) target, located 2.1 km underground at SNOLAB. The experimental signature of dark matter interactions is keV-scale $^{40}$Ar nuclear recoils (NR) producing 128 nm LAr scintillation photons observed by PMTs. The largest backgrounds in DEAP-3600 are electronic recoils (ER) induced by $\beta$ and $\gamma$-rays originating from internal and external radioactivity in the detector material. A background model of the ER interactions in DEAP-3600 was developed and is described in this work. The model is based on several components which are expected from radioisotopes in the LAr, from ex-situ material assay measurements, and from dedicated independent in-situ analyses. This prior information is used in a Bayesian fit of the ER components to a 247.2 d dataset to model the radioactivity in the surrounding detector materials. While excellent discrimination between ERs and NRs is reached with pulse shape discrimination, utilizing the large difference between fast and slow components of LAr scintillation light, detailed knowledge of the ER background and activity of detector components, sets valuable constraints on other key types of backgrounds in the detector: neutrons and alphas. In addition, the activity of $^{42}$Ar in LAr in DEAP-3600 is determined by measuring the daughter decay of $^{42}$K. This cosmogenically activated trace isotope is a relevant background at higher energies for other rare event searches using atmospheric argon e.g. DarkSide-20k, GERDA or LEGEND. The specific activity of $^{42}$Ar in the atmosphere is found to be $40.4 \pm 5.9$ $\mu$Bq/kg of argon.

==> detector.tex <==
\subsection{Experimental Setup}
\label{sec:ExperimentalSetup}


\textcolor{blue}{CJJ: detector section starts here.}  For the data set
DEAP-3600 consists of $3256\pm 110$~kg of LAr in a 5~cm thick acrilyc sphere of
radius 85~cm. The inner surface of the sphere is coated with a
3~$\mu$m thick layer of 1,1,4,4-tetraphenyl-1,3-butadiene (TPB), an
organic wavelength shifter which absorbs the 128~nm scintillation
light and emits in a distribution peaked at 420~nm.

Light is observed by 255 Hamamatsu R5912 HQE PMTs that are mounted
with an oil coupling to 50~cm long acrylic light guides (LGs) that are
bonded to the sphere. There is excellent optical transmission from the
TPB to the PMTs. The space between the LGs is filled with blocks 
of alternating HDPE and polystyrene layers. These filler blocks (FBs)
and LGs provide excellent neutron and \gray\ shielding. They also
support a thermal gradient between the cold LAr and the PMTs
that are operated at -20~C.

The detector is surrounded by a ASMI Section VIII pressure vessel (the
stainless steel shell, SSS) that is 3.4~m in diameter and 9.5~mm
thick. The SSS is suspended in a cylindrical water tank with a 7.8~m
height and diameter.

The argon was purified in gas phase during fill using a SAES getter
and a custom charcoal radon trap. The argon is cooled with a coil in
the neck of the detector which through which liquid nitrogen is
flowed. The neck introduces an asymmetry in the detector. Once the
detctor was filled, it was sealed for the duration of the data set
(and beyond). 

The data aquisition was designed to handle the high rates of events
from \nuc{Ar}{39}, be sensitive at low energy to WIMPs and allow
thorough investigation of backgrounds. The signals from the 255 argon
PMT are amplified in custom boards and read out by 12-bit 250~MS/s
CAEN V1720 digitizers. For nomal data taking, the digitizers are  operated with
zero-length encoding (ZLE, ie zero suppression) to reduce data
volume and a custom trigger initiates recording of data using using the
total measured light in a window and pulse shape (using a 177~ns and a
3100~ns window). The trigger prescales by a factor of 100 the low \fp
events with an energy higher than the WIMP search region to
approximately the endpoint of \nuc{ar}{39}. For each event, PMT signals are recorded
over 16~$\mu$s starting about 2.5~$\mu$s before the trigger time.
Data are organized into runs with a run time of $\simeq 1$~hr to $\simeq 1$~day.
Details are available in \cite{DEAPDetector}.

PMT calibrations are carried out daily using injection of visible light
by optical fibres. Periodic detector calibrations are carried out
\nuc{Na}{22}, \nuc{U}{232}, and \nuc{AmBe}{241} sources deployed in
guide tubes outside the SSS. Normal running allows for run-by-run
calibration with \nuc{Ar}{39} and background \glines\ from
\nuc{Tl}{208} and \nuc{K}{40}.





